Dirichlet-based Uncertainty Quantification for Personalized Federated Learning with Improved Posterior Networks

In modern federated learning, one of the main challenges is to account for inherent heterogeneity and the diverse nature of data distributions for different clients. This problem is often addressed by introducing personalization of the models towards the data distribution of the particular client. However, a personalized model might be unreliable when applied to the data that is not typical for this client. Eventually, it may perform worse for these data than the non-personalized global model trained in a federated way on the data from all the clients. This paper presents a new approach to federated learning that allows selecting a model from global and personalized ones that would perform better for a particular input point. It is achieved through a careful modeling of predictive uncertainties that helps to detect local and global in- and out-of-distribution data and use this information to select the model that is confident in a prediction. The comprehensive experimental evaluation on the popular real-world image datasets shows the superior performance of the model in the presence of out-of-distribution data while performing on par with state-of-the-art personalized federated learning algorithms in the standard scenarios.

==> neurips_2023/conclusion.tex <==
% !TEX root = main.tex

\section{Conclusion}
\label{sec:conclusion}

In this paper, we proposed a personalized federated learning framework that leverages both a globally trained federated model and personalized local models to make final predictions. The selection between these models is based on the confidence in the prediction. 

Our empirical evaluation demonstrated that, under realistic scenario, this approach outperforms both local and global models when used independently. While the model's capacity to handle out-of-distribution data is not perfect and depends on various factors, such as the quality of the global model and the selection of the threshold, our ``switching'' approach ultimately leads to improved performance. It also enhances the reliability of AI applications, underscoring the potential of our methodology in a broader context of federated learning environments


==> neurips_2023/def.tex <==
\newcommand{\R}{\mathbb{R}}

\newcommand\TODO[1]{\textcolor{red}{#1}}
\newcommand{\Dtr}{ D_\texttt{tr} }
\newcommand{\aprior}{ \boldsymbol\alpha^\text{prior} }
\newcommand{\apriorc}{ \alpha^\text{prior} }

\newcommand{\apost}{ \boldsymbol\alpha^\text{post} }
\newcommand{\apostc}{ \alpha^\text{post} }

\newcommand{\al}{ \boldsymbol\alpha }


\newcommand{\muv}{ \boldsymbol\mu }
\newcommand{\yv}{ \boldsymbol y }
\newcommand{\dirpost}{ \textit{Dir}\bigl(\muv \mid \apost(x)\bigr)}
\newcommand{\dirplain}{ \textit{Dir}\bigl(\muv \mid \al(x)\bigr)}

\newcommand{\smmodel}{ \boldsymbol f }
\newcommand{\embedmodel}{ g }

\newcommand{\indicator}{ \mathds{1} }
\newcommand{\E}{ \mathbb{E} }
\newcommand{\entropy}{ \mathcal{H} }


==> neurips_2023/experiments.tex <==
% !TEX root = main.tex

\section{Experiments}
\label{sec:experiments}
  In this section, we assess the effectiveness of our proposed method through a series of thorough experiments. 
  We employ seven diverse datasets: MNIST~\cite{lecun1998mnist}, FashionMNIST~\cite{xiao2017fashion}, MedMNIST-A, MedMNIST-C, MedMNIST-S~\cite{medmnistv1,medmnistv2}, CIFAR10~\cite{krizhevsky2009learning}, and SVHN~\cite{netzer2011reading}. The LeNet-5~\cite{lecun1998gradient} encoder architecture is applied to the first five datasets, while ResNet-18~\cite{he2016deep} is used for CIFAR10 and SVHN. Building on the ideas from~\cite{charpentier2020posterior, charpentier2021natural}, we implemented the Radial Flow~\cite{rezende2015variational} normalizing flow due to its lightweight nature and inherent flexibility.
  In all our experiments, we focus on a heterogeneous data distribution across clients. We consider a scenario involving 20 clients, each possessing a random subset of 2 or 3 classes. However, the overall amount of data each client possesses is approximately equal. The federated learning process is conducted using \texttt{FedAvg} algorithm.

  In the following sections, we present different experiments that highlight the strengths of our approach. We should note that we don't have a dedicated experiment to illustrate how approach deals with local ambiguous data as the vision datasets we are considering have actually very few points of this type.

\subsection{Threshold selection}
  Before discussing the results, it is essential to understand how we determine whether to make predictions using a local model or a global one.

  This decision, resulting in a ``switching'' model, depends on a particular uncertainty score. This score can either be the logarithm of the density of embeddings, obtained using the density model (normalizing flows), or the entropy of predictive Dirichlet distribution~\eqref{eq:entropy}. We found that both measures provide comparable behaviour, and in the experiments for the Table~\ref{tab:switching_accuracy} we use density of embeddings, while for the Table~\ref{tab:ood_accuracy} we use Dirichlet entropy.

  To apply this approach, we must establish a rule for how a client decides whether to use its local model for predictions on a previously unseen input object $x$ or to delegate the prediction to the global model.
  One approach is to select some uncertainty values' threshold. This threshold can be chosen based on an additional calibration dataset. In our experiments, we split each client's validation dataset in a 40/60 ratio, using the smaller part for calibration.
  Note that the calibration dataset only includes those classes used during the training procedure.

  The choice of the threshold is arguably the most subjective part of the approach. Ideally, we would desire to have access to explicit out-of-distribution data (either from other client ``local OOD'' or completely unrelated data ``global OOD''). With this data, we could explicitly compute uncertainty scores for both types of data (in-distribution and out-of-distribution) and select the threshold that maximizes accuracy.
  However, we believe it is unfair to assume that we have this data in the problem statement. Therefore, we suggest a procedure for choosing the threshold based solely on available local data.

  To choose the threshold, we assume that for all clients, there might be a chance that some \(p\%\) (typically 10\%) of objects are actually outliers. We further compute the estimates of epistemic uncertainty (with either entropy or the logarithms of density of embeddings) and select an appropriate threshold based on this assumption. 
  % Then, for the \textbf{remaining points of the calibration set}, we can compute the threshold on aleatoric uncertainty that maximizes the prediction quality on the low uncertainty points.
  % \nk{I did not get, what are these remaining points?}
  %
  For the high epistemic uncertainty points of the global model, a similar thresholding can be performed to optimize its prediction quality. %of a global model.
  %\mti{why not to compute threshold in a way, that we feed 5\% of random data / different data, and take the 5\% quantile for the confident scores??}


\subsection{Assessing performance of the switching model}
\label{sec:switching_performance}
  % \begin{table}[t!]
  %   \centering
  %   \resizebox{\textwidth}{!}{
  %   \begin{tabular}{@{}l|lll|lll|lll@{}}
  %     \toprule
  %     Dataset  & \multicolumn{3}{c}{InD}                & \multicolumn{3}{c}{OOD}  
  %             & \multicolumn{3}{c}{Mix}  \\ \midrule
  %     Model & Local & Global & Switch & Local & Global & Switch & Local & Global & Switch \\ \midrule
  %     MNIST & $99.7 \pm 0.2$ & $98.0 \pm 0.7$ & $98.4 \pm 0.4$ & $0.0 \pm 0.0$ & $98.1 \pm 0.3$ & $97.7 \pm 0.3$ & $49.8 \pm 0.1$ & $98.0 \pm 0.2$ & $98.0 \pm 0.2$ \\
  %     FashionMNIST & $97.7 \pm 2.9$ & $63.6 \pm 23.5$ & $85.5 \pm 8.8$ & $0.0 \pm 0.0$ & $69.1 \pm 7.3$ & $61.8 \pm 7.5$ & $48.9 \pm 1.4$ & $66.3 \pm 8.3$ & $73.7 \pm 3.0$ \\
  %     MedMNIST-A & $97.1 \pm 2.8$ & $65.5 \pm 17.6$ & $83.6 \pm 7.4$ & $0.9 \pm 1.2$ & $67.2 \pm 6.0$ & $59.8 \pm 6.8$ & $49.3 \pm 1.9$ & $63.9 \pm 6.3$ & $69.5 \pm 3.4$ \\
  %     MedMNIST-C & $81.6 \pm 11.1$ & $55.2 \pm 17.4$ & $71.9 \pm 11.0$ & $2.2 \pm 2.7$ & $59.8 \pm 6.0$ & $34.1 \pm 17.3$ & $41.8 \pm 6.0$ & $textbf{54.6} \pm 6.9$ & $53.2 \pm 9.4$ \\
  %     MedMNIST-S & $85.1 \pm 13.2$ & $43.2 \pm 27.4$ & $64.6 \pm 15.2$ & $0.1 \pm 0.2$ & $50.2 \pm 9.7$ & $29.5 \pm 12.9$ & $42.7 \pm 6.6$ & $39.7 \pm 10.8$ & $textbf{43.7} \pm 7.4$ \\
  %     CIFAR10 & $90.0 \pm 10.9$ & $30.8 \pm 21.3$ & $67.6 \pm 10.0$ & $0.1 \pm 0.1$ & $29.5 \pm 6.7$ & $26.9 \pm 6.3$ & $45.0 \pm 5.5$ & $30.1 \pm 7.5$ & $textbf{47.2} \pm 4.2$ \\
  %     SVHN & $95.9 \pm 1.8$ & $36.0 \pm 32.4$ & $84.5 \pm 8.0$ & $0.9 \pm 1.3$ & $32.0 \pm 10.4$ & $29.2 \pm 10.1$ & $48.6 \pm 1.3$ & $37.2 \pm 11.3$ & $\textbf{59.8} \pm 3.8$ \\
  %     \bottomrule
  %   \end{tabular}
  %   }
    
  %   \caption{The table presents the average (per-client) predictive accuracy of various models, segmented according to the client's training distribution. The data is partitioned into three sets: InD (comprising only the classes seen during training), OOD (all other classes), and Mix (a combination of both, representing the entire data domain). It is evident from the table that alternating between the local and global models based on the model confidence helps enhance the predictive performance of both models in the most realistic scenario represented by the Mix set (third column).}
  % \label{tab:switching_accuracy}
  % \end{table}


      %   \begin{tabular}{@{}l|lll|lll|lll@{}}
      %   \toprule
      %         & \multicolumn{3}{c}{InD}                & \multicolumn{3}{c}{OOD}  
      %         & \multicolumn{3}{c}{Mix}  \\ \midrule
      %   Dataset & Local & Global & Switch & Local & Global & Switch & Local & Global & Switch \\ \midrule
      %   MNIST & 99.7 & 98.0 & 98.4 & 0.0 & 98.1 & 97.7 & 49.8 & \textbf{98.0} & \textbf{98.0} \\
      %   FashionMNIST & 97.7 & 63.6 & 85.5 & 0.0 & 69.1 & 61.8 & 48.9 & 66.3 & \textbf{73.7} \\
      %   MedMNIST-A & 97.1 & 65.5 & 83.6 & 0.9 & 67.2 & 59.8 & 49.3 & 63.9 & \textbf{69.5} \\
      %   MedMNIST-C & 81.6 & 55.2 & 71.9 & 2.2 & 59.8 & 34.1 & 41.8 & \textbf{54.6} & 53.2 \\
      %   MedMNIST-S & 85.1 & 43.2 & 64.6 & 0.1 & 50.2 & 29.5 & 42.7 & 39.7 & \textbf{43.7} \\
      %   CIFAR10 & 90.0 & 30.8 & 67.6 & 0.1 & 29.5 & 26.9 & 45.0 & 30.1 & \textbf{47.2} \\
      %   SVHN & 95.9 & 36.0 & 84.5 & 0.9 & 32.0 & 29.2 & 48.6 & 37.2 & \textbf{59.8} \\
      %   \bottomrule
      % \end{tabular}

  \begin{table}[t!]
    \centering
    \resizebox{0.9\textwidth}{!}{
      \begin{tabular}{@{}l|lll|lll|lll@{}}
        \toprule
              & \multicolumn{3}{c}{InD}                & \multicolumn{3}{c}{OOD}  
              & \multicolumn{3}{c}{Mix}  \\ \midrule
        Dataset & Local & Global & Switch & Local & Global & Switch & Local & Global & Switch \\ \midrule
        MNIST & 99.4 & 98.3 & 98.4 & 0.0 & 98.3 & 98.3 & 49.7 & \textbf{98.3} & \textbf{98.3} \\
        FashionMNIST & 95.7 & 80.0 & 85.2 & 0.0 & 81.5 & 77.1 & 47.9 & 80.7 & \textbf{81.2} \\
        MedMNIST-A & 99.0 & 95.9 & 96.4 & 0.0 & 95.2 & 94.6 & 49.6 & \textbf{95.5} & \textbf{95.5} \\
        MedMNIST-C & 96.6 & 93.9 & 94.6 & 0.0 & 93.1 & 87.1 & 48.4 & \textbf{93.2} & 90.5 \\
        MedMNIST-S & 90.7 & 83.0 & 87.2 & 0.0 & 82.7 & 73.2 & 45.4 & \textbf{81.4} & 79.3 \\
        CIFAR10 & 75.1 & 39.6 & 60.1 & 0.0 & 38.8 & 27.9 & 37.6 & 39.4 & \textbf{44.1} \\
        SVHN & 92.2 & 77.8 & 88.9 & 0.0 & 77.5 & 49.1 & 46.1 & \textbf{76.2} & 67.9 \\
        \bottomrule
      \end{tabular}
    }
    \caption{The table presents the average (per-client) predictive accuracy of various models, segmented according to the client's training distribution. The data is partitioned into three sets: InD (comprising only the classes seen during training), OOD (all other classes), and Mix (a combination of both, representing the entire data domain). It is evident from the table that alternating between the local and global models based on the model confidence helps enhance the predictive performance of both models in the most realistic scenario represented by the Mix set (third column). For the Mix set the best performing method is in \textbf{bold}.}
  \label{tab:switching_accuracy}
  \end{table}

  In this section, we assess the performance of our method, where the prediction alternates between local and global models based on the uncertainty threshold.

  For each dataset, we trained three types of models. First, a global model is trained as a result of the federated procedure, following \texttt{FedAvg} procedure. 
  Then, every client, after the federated procedure, retains the resulting encoder network while the classifier and flow are retrained from scratch using only local data.
  The third type of model, the ``switching'' model, alternates between the first two models based on the uncertainty threshold set for each client.

  Additionally, for each client, we consider the following three types of data: data of the same classes used during training (InD), data of all other classes (OOD), and data from all classes (Mix). For each of these models, datasets, and data splits, we compute the average prediction accuracy (client-wise). % along with the standard deviations. 
  The results of this experiment are presented in Table~\ref{tab:switching_accuracy}.

  From the Table~\ref{tab:switching_accuracy}, we observe that the ``switching'' model's performance for InD data is always better than the one for the global model though inferior to the local one. 
  %In scenarios where the out-of-distribution domain is known, a more accurate threshold selection is possible.
  For the OOD data, it is evident that the ``switching'' model improves over the local model's performance. This situation corresponds to the ``local OOD (unknown knowns)'' case from Table~\ref{table:example}, illustrating the benefits of referring to global knowledge when the local model is unfamiliar with the data.
  The third column illustrates a scenario where the input data includes whole domain of the training data. This is the most realistic practical scenario — all the clients aim to collaboratively solve the same problem, given different local data. However, due to the heterogeneous nature of the between-clients data distribution (covariate shift), local models cannot learn the entire data manifold.
  Therefore, occasionally referring to global knowledge is beneficial while still preserving personalization when the local model is confident. We observe that the ``switching'' model outperforms both local and global models on 6 datasets out of 8 while showing the same performance with the global model on MNIST.

  %In the next section, we will study our method's behavior in the presence of both -- ``soft-OOD'' (unknown knowns or local OOD) and ``hard OOD'' (unknown unknowns or global OOD).

  % While this experiment examined our method's behavior in the presence of ``soft-OOD'' or unknown-known data, it is also interesting to explore how the method operates in the presence of ``hard-OOD'' or unknown-unknown situations.


\subsection{Assessment in the presence of global out-of-distribution (unknown-unknown) data}
  %In this section we study how effectively the models, trained under our framework, distinguish between in-distribution and out-of-distribution data.
  In this section, we will study our method's behavior in the presence of both -- ``soft-OOD'' (unknown knowns or local OOD) and ``hard OOD'' (unknown unknowns or global OOD).

  We suggest the following experimental setup. 
  %We start our study by determining the threshold for each local model using its respective calibration data.
  Subsequently, we identify a pair of datasets -- the first is the entire InD dataset, fragments of which were distributed among federated clients during training. The second dataset represents explicit OOD data, unassociated with the federated training procedure.
  Our primary objective is to evaluate the performance of our models when faced with various types of data. We propose the following scheme to achieve this. 

  Firstly, both datasets are fed into the local model which, based on the predetermined threshold, labels each input as either in-distribution or out-of-distribution. %As we know the correct origin for each training object, we can assess the accuracy of this labeling. Note that for local models, any objects not part of the training classes are considered out-of-distribution. The average accuracy of this labeling, calculated across all clients, is reported in Table~\ref{tab:ood_accuracy}.
  Subsequently, the local model makes prediction for the objects classified as in-distribution by it, and the remaining objects are further processed by the global model.
  
  The process of selecting a threshold for the global model is arguably even more complex than for the local model. In practice it might be determined based either on a local data of each particular client or possibly based on the separate global calibration data. In our experiments we consider varying this threshold in order to evaluate how the model's performance metric depend on the fraction of filtered objects. As a quality measure we consider the precision of predictions of the model for a given client. Apparently, we expect that if we filter OOD objects well, then the precision improves with the fraction of filtered objects as we obtain less false positives. %Since each client only retains the weights without any data collected from other clients, we are compelled to use the local calibration dataset (comprising only a subset of classes) to determine the threshold.
  % With this threshold established, we once again categorize the remaining objects as either in-distribution or out-of-distribution, and compute the resulting accuracy.
  % Finally, we exclude those objects marked as in-distribution by the global model. For the remaining objects, we assign a uniform prediction of ``all are out-of-distribution'' and calculate the resulting accuracy.

  First, on Figure~\ref{fig:ood_plot} we show how for the task with InD MNIST dataset and OOD FashionMNIST precision improves with increased fraction of the filtered data. It shows that the considered uncertainty metric filters well uncertain objects thus improving the performance. Then, in Table~\ref{tab:ood_accuracy}, we present the average increase in precision when 50\%for the considered datasets. We note that we had 50\% of OOD samples in the data and, thus, in the ideal case we filter out all the OOD data for the selected threshold. We clearly observe the significant increase in precision over all the datasets. Some additional experimental results for this experiment can be found in SM.


      %   \begin{tabular}{@{}lll@{}}
      %   \toprule
      %   In-distribution & Out-of-distribution & Prec. impr. \\ \midrule
      %   MNIST           & FashionMNIST        & 42.01                 \\
      %   FashionMNIST    & MNIST               & 28.34                 \\
      %   CIFAR10         & SVHN                & 27.94                 \\
      %   SVHN            & CIFAR10             & 41.52                 \\
      %   MedMNIST-A      & FashionMNIST        & 26.88                 \\
      %   MedMNIST-S      & FashionMNIST        & 15.57                 \\
      %   MedMNIST-C      & FashionMNIST        & 11.60                 \\ \bottomrule
      % \end{tabular}

  \begin{figure}[t!]
    \centering
    \begin{minipage}{0.45\textwidth}
      \includegraphics[width=1\textwidth]{pics/mnist_precision.pdf}
      \captionof{figure}{This graph illustrates the variation in precision as a function of the filtering threshold for MNIST InD data and FashionMNIST OOD data}
    \label{fig:ood_plot}
    \end{minipage}
    \begin{minipage}{0.54\textwidth}
      \begin{tabular}{@{}lll@{}}
        \toprule
        In-distribution & Out-of-distribution & Prec. impr. \\ \midrule
        MNIST           & FashionMNIST        & 53.15                 \\
        FashionMNIST    & MNIST               & 59.03                 \\
        CIFAR10         & SVHN                & 38.68                 \\
        SVHN            & CIFAR10             & 19.02                 \\
        MedMNIST-A      & FashionMNIST        & 38.67                 \\
        MedMNIST-S      & FashionMNIST        & 14.27                 \\
        MedMNIST-C      & FashionMNIST        & 14.44                 \\ \bottomrule
      \end{tabular}
      \captionof{table}{The table shows improvement (in percentage) of precision, given that 50\% of the objects were filtered by their uncertainty, evaluated using global model.}
      \label{tab:ood_accuracy}
    \end{minipage}

  \end{figure}
  % \begin{table}[t!]
  %   \centering
  %   \begin{tabular}{@{}ll|lll@{}}
  %   \toprule
  %   InD dataset  & OOD dataset  & Loc.  & Glob. & OOD   \\ \midrule
  %   MNIST        & FashionMNIST & 85.4 & 92.5 & 94.6 \\
  %   FashionMNIST & MNIST        & 78.1 & 65.3 & 71.6   \\
  %   CIFAR10         & SVHN      & 88.2 & 50.3  & 61.9 \\
  %   SVHN         & CIFAR10      & 70.5 & 49.5  & 37.3 \\
  %   MedMNIST-A   & FashionMNIST & 73.4 & 69.8 & 75.0   \\
  %   MedMNIST-S   & FashionMNIST & 55.6  & 45.3  & 70.1   \\
  %   MedMNIST-C   & FashionMNIST & 48.9  & 28.9 & 42.8   \\ \bottomrule
  %   \end{tabular}
  %   \caption{Accuracy of identifying in-distribution and out-of-distribution data, determined by the chosen thresholds.}
  % \label{tab:ood_accuracy}
  % \end{table}

  %It can be observed that the global model's decision-making is less certain for the CIFAR10 and SVHN datasets. This can be attributed to two factors. Firstly, the process of choosing the threshold for this model isn't well defined. Given that the global model has ``encountered'' all the data, it seems inefficient to select a threshold based on the incomplete local calibration data (only a subset of classes). Secondly, due to data heterogeneity, the global model itself does not perform optimally for these datasets (see Table~\ref{tab:switching_accuracy}), which could lead to ambiguous embeddings of the classes used for uncertainty quantification.


==> neurips_2023/framework.tex <==
% !TEX root = main.tex

\section{General framework of switching between global and personal models}
\label{sec:method}
  \begin{wrapfigure}{r}{0.5\textwidth}
    \vspace{-20pt}

    \centering
    \includegraphics[width=0.5\textwidth]{pics/diagram_approach.png}
    \caption{The general scheme of the proposed approach. Each input is first processed by personalized local model. In case of high epistemic uncertainty, the decision is delegated to the global model. Otherwise, if epistemic uncertainty is low, local model proceeds with the decision. Both models consider also aleatoric uncertainty and may abstain from prediction.
    }

    \vspace{-30pt}
  \label{fig:main_scheme}
  %\mti{do we want to put more details in the caption?}
  \end{wrapfigure}

  In this section, we introduce our framework, discussing the general idea and potential nuances. In the subsequent section, we will delve into a specific implementation.

\subsection{Concept overview}
  We are going to consider a federated learning setting with multiple clients, each having its own personalized local model. However, we additionally assume that the global model is available. The global model is typically expected to perform reasonably well on each client's data. Assuming that we already have trained global and local models, we consider a situation where clients have the option to use either the global model or their local model to make predictions for a new unseen object $x$. 

  The choice between local and global model for prediction depends on the multiple factors that contribute to their prediction quality. First of all, shift in the distribution between the local data of a particular client and the global population may have significant effect on the models' performance. Possible shifts include covariate shift, label shift or different types of label noise. If the shift is significant, the global model might be very biased with respect to the prediction for the particular client, while normally the local model is unbiased. The second part of the picture is the size of the available data. Generally, the global model has more data and potentially, if no data shift is present, should outperform the local one. However, the global model is usually trained with no direct access to the data stored at clients, which might degrade its performance. Eventually, the best performing model will be the one which achieves better bias variance trade-off.

  In this work, we propose a framework to choose between pointwise usage of local or global model for prediction based on the uncertainty scores provided by the model (or abstain from making a prediction altogether, explicitly acknowledging the uncertainty). We assume that both local and global models can provide uncertainty estimates corresponding not only to the total predictive uncertainty but also to separately aleatoric and epistemic uncertainties. %~\todo{we need to expand here or above explaining the uncertainties}. 
  The resulting workflow is summarized in Figure~\ref{fig:main_scheme}.


\subsection{Optimal choice of model}
  We start from the important fact that the local model is not exposed to the data shift between the general population and the particular client. Thus, if this model is sufficiently confident in the prediction, there is no need to involve the global model at all. However, it is important to distinguish between different types of uncertainty here. Usually, the total uncertainty of the model predicting at a particular data point can be split into two parts: aleatoric uncertainty and epistemic uncertainty~\cite{hullermeier2021aleatoric}. \textit{Aleatoric} uncertainty is the one that reflects the inherent noise in the data. The epistemic uncertainty is the one that reflects the lack of knowledge due to the fact that the model was trained on a data set of a limited size. 

  For our problem, it is extremely important to distinguish between aleatoric and epistemic uncertainties. Suppose the local model has low epistemic and high aleatoric uncertainty at some point. In that case, the model is confident that the predicted label is ambiguous, and the model should abstain from prediction. However, if the epistemic uncertainty is high, it means that the model doesn't have enough knowledge to make the prediction (not enough data), and the global model should make the decision. The global model, in its turn, may either proceed with the prediction if it is confident or abstain from prediction if there is high uncertainty associated with the prediction. Thus, in this context, for a fixed client and an unseen input, there are four possible outcomes, see Table~\ref{table:example}.

  \begin{table}[t!]
    \centering
    \begin{tabular}{|>{\centering\arraybackslash}m{0.45\linewidth}|>{\centering\arraybackslash}m{0.45\linewidth}|}
      \hline
      \textbf{Known knowns} & \textbf{Known unknowns} \\
      \small{\textbf{Local Confident.} This represents local in-distribution data for which the local model is confident in prediction.} & \small{\textbf{Local Ambiguous.} 
      This is local in-distribution data with high aleatoric uncertainty (class ambiguity). 
      % Since the global model might exhibit higher aleatoric uncertainty in this area, we will still use the local model for predictions.
      } \\
      \hline
      \textbf{Unknown knowns} & \textbf{Unknown unknowns} \\
      \small{\textbf{Local OOD.} This refers to data that is locally unknown (high epistemic uncertainty) but known to other clients. In this case, it makes sense to use the global model for predictions.} & \small{\textbf{Global Uncertain.} These input data is out-of-distribution for the local model while the global model is uncertain in prediction (high total uncertainty). The best course of action is to abstain from making a prediction.} \\
      \hline
    \end{tabular}
    \caption{Possible scenarios for the input data point in the introduced setup. A particular input falls in one of the categories depending on the confidence in its prediction by local and global models. The disentanglement between aleatoric and epistemic uncertainties is crucial to make the decision in an optimal way.}
  \label{table:example}
  \end{table}

  % In this section we discuss the rule, how a client indexed $i$, having its local parameters of flow $\psi_i$ and head $\theta_i$ can choose whether to use it for the predictions on unseen input object $x$, or to delegate the prediction to the global model.

  %Subsequently, for any new unseen input, we compute the same uncertainty metric (using local model) and compare it with the threshold. If the metric exceeds the threshold, we delegate the prediction to the global model; otherwise, we predict locally.

  %\TODO{NK: Can we do (and do we really need?) the same test for the global model to abstain from making a prediction? Because calibration datasets for all the clients are different, and due to all these heterogeneity/personalization, it does not seem straightforward.}

  %It is essential to emphasize that our decision-making process starts with the local model rather than the global one.
  %The intuition behind this idea is that the local model, having been trained on the client's own data, does not exhibit bias due to heterogeneity as the global model might.
  %Furthermore, the local model is inherently tailored to the specific client, whereas the global one is not.
  %Consequently, initiating our consideration from this ``flawless'' model allows us to make the most informed and accurate decisions within our framework. 
  %By prioritizing the local model in this manner, we can ensure a more nuanced and precise understanding of the data, leading to improved overall performance.

  %\TODO{NK: I want to prove theoretically that the rule based on uncertainty scores/embedding density is optimal in some sense.}

  The particular implementation of the approach described above would depend on the choice of the machine learning model and the way to compute uncertainty estimates. The key feature required is the ability of the method to compute both aleatoric and epistemic uncertainties. In the next section, we propose the implementation of the method based on the posterior networks framework~\cite{charpentier2020posterior}.


==> neurips_2023/introduction.tex <==
% !TEX root = main.tex

\section{Introduction}
\label{sec:intro}
  The widespread adoption of deep neural networks in various applications requires reliable predictions, which can be achieved through rigorous uncertainty quantification. Although uncertainty quantification has been extensively studied in different domains under centralized settings~\cite{NEURIPS2018_abdeb6f5, lakshminarayanan2017simple, gal2016dropout, kotelevskii2022nonparametric}, only a few works have considered this area within the context of federated learning~\cite{kotelevskii2022fedpop, linsner2022approaches}. Typically, in federated learning papers, algorithms result in using either a personalized local model or a global model. However, both these models could be useful in different cases by providing the tradeoff between personalization of a local model and higher reliability of the global one~\cite{hanzely2020federated,liang2020think}.

  In this paper, we introduce a new framework to choose whether to predict with a local or global model at a given point based on uncertainty quantification. The core idea is to apply the global model only if the local one has high epistemic (model) uncertainty~\cite{hullermeier2021aleatoric} about the prediction at a given point, i.e., the local model doesn't have enough information about the particular input point. In case the local model is confident (either in predicting a particular class or in the fact that it is observing an ambiguous object with high aleatoric (data) uncertainty~\cite{hullermeier2021aleatoric}), it should make the decision itself without involving the global one.  %The problem of uncertainty quantification has been extensively studied in numerous centralized scenarios across various data domains. However, the application of this topic to federated learning has not yet been thoroughly investigated. While some attempts have been made to quantify uncertainty in federated settings, such as in~\cite{linsner2022approaches, kotelevskii2022fedpop}, these studies neither differentiate between aleatoric and epistemic uncertainties nor provide practical solutions.
  
  As a specific instance of our framework, we propose an approach inspired by Posterior Networks (\texttt{PostNet})~\cite{charpentier2020posterior} and its modification, Natural Posterior Networks (\texttt{NatPN})~\cite{charpentier2021natural}. This type of model is particularly useful for our purposes, as it enables the estimation of aleatoric and epistemic uncertainties without incurring additional inference costs. Thus, we are able to fully implement the switching between local and global models in an efficient way.
  
  \paragraph{Related work.} In~\cite{linsner2022approaches}, the authors suggest training an ensemble of $K$ global models as the best approach for federated uncertainty quantification, which is $K$ times more expensive compared to the classical \texttt{FedAvg} method. In~\cite{kotelevskii2022fedpop}, the authors propose using Markov Chain Monte Carlo (MCMC) to obtain samples from the posterior distribution, which is practically almost infeasible due to its computational complexity.

  Other works, such as~\cite{chen2020fedbe, kimhierarchical}, could potentially be utilized for estimating uncertainty in federated learning. However, these studies do not explicitly discuss the opportunities and challenges associated with uncertainty quantification in their papers.

  The central idea of \texttt{PostNet} and \texttt{NatPN} involves using a Dirichlet prior and posterior distributions over the categorical predictive distributions~\cite{malinin2018predictive, malinin2019reverse, charpentier2020posterior, charpentier2021natural, sensoy2018evidential}. To parameterize the parameters of these Dirichlet distributions, the authors suggest introducing a density model over the deep representations of input objects. In \texttt{NatPN}, a Normalizing Flow~\cite{papamakarios2021normalizing, kobyzev2020normalizing} is employed to estimate the density of embeddings extracted by a trained feature extractor. This density is then used to calculate updates to the Dirichlet distribution.

  Despite the success of the \texttt{NatPN} model~\cite{charpentier2021natural}, we identified certain issues with the loss function employed in \texttt{NatPN}, which become particularly critical when dealing with high aleatoric regions (which could be a potential issue in federated learning). Intriguingly, the issue was not discovered in the authors' recent work~\cite{charpentier2023training}, which investigated potential issues in the training procedure. Recent works~\cite{bengs2022pitfalls, bengs2023second} have unveiled other potential issues related to the training of Dirichlet models in general but have not offered solutions to address these challenges.

\paragraph{Contributions.}
  Our paper stands out as one of the few studies that specifically addresses the problem of uncertainty quantification in federated learning. We aim to provide a comprehensive analysis of this important topic, considering both theoretical and practical aspects, and presenting solutions that overcome the limitations of existing approaches in the literature. The contributions of this paper are as follows:
  \begin{enumerate}
    \item We present the first framework in federated learning based on uncertainty quantification, which allows switching between using a local or global model. We introduce the definitions of \textit{Local-Confident}, \textit{Local-Ambiguous}, \textit{Local-OOD}, and \textit{Global-Uncertain} -- helpful concepts that enable us to reason about the choice of model for prediction.

    \item We introduce a specific realization of our framework \texttt{FedPN}, using Dirichlet-based \texttt{NatPN} model. For this particular model, we identify an issue in the loss function of \texttt{NatPN} (not known in literature before) that complicates disentanglement of aleatoric and epistemic uncertainties, and propose a solution to rectify it.

    %\item \TODO{We provide a simple, provably optimal rule for determining which model (global or local) to use when making predictions for a given unseen object.}

    \item We conduct an extensive set of experiments that demonstrate the benefits of our approach for different input data scenarios.
  \end{enumerate}

  % By addressing the challenges in uncertainty quantification for federated learning, our work aims to improve the reliability and applicability of federated learning models. The proposed framework, along with the specific realization using NatPN, provides a flexible and effective solution for deciding between local and global models based on uncertainty quantification. Our identification and rectification of the loss function issue in NatPN, as well as the provably optimal rule for model selection, further strengthen the practicality of our approach. Ultimately, the extensive experimental results validate the effectiveness of our framework in handling various input data scenarios, showcasing its potential for real-world applications.


==> neurips_2023/method.tex <==
% !TEX root = main.tex

\section{Dirichlet-based deep learning models}
\label{sec:background}
  We have chosen to showcase Dirichlet-based models~\cite{malinin2018predictive,charpentier2020posterior,charpentier2021natural} as a specific instance of our general framework.
  The intuition behind this decision lies in the fact that these models allows the distinction between various types of uncertainty and facilitate the computation of corresponding uncertainty estimates with minimal additional computational overhead.
  Furthermore, unlike ensemble methods~\cite{beluch2018power}, there is no need to train multiple models.
  In comparison to approximate Bayesian techniques, such as MC Dropout~\cite{gal2016dropout} or Variational Inference~\cite{graves2011practical}, almost all expectations of interest can be derived in closed form.
  This makes Dirichlet-based models an attractive and efficient option for implementing our proposed framework.

  % However, to the best our knowledge, normalizing flows were not studied in application to federated learning. It is not clear how to optimize it, especially when the data between clients is highly heterogeneous.

  % Inspired by FedAvg~\cite{mcmahan2017communication} optimization procedure, we assume that averaging models weights, received from clients, also provides reasonable results for Normalizing flows.

  % Ultimately, we would like to build a model, which benefits from both worlds -- personalized federated learning and not-personalized.
  % Personalization is good, when data is heterogeneous, but also when a client has a sufficient amount of data to learn reasonable parameters and to perform good inference.
  % However, when it is not the case (in other words an input object is local out-of-distribution), we might want to resort to global model prediction.
  % But if an input object is complete out-of-distribution, than we would like to produce maximum-entropy prediction, whatever task we are solving (uniform posterior predictive distribution in case of Categorical likelihood, Standard Gaussian for normal likelihood etc).


\subsection{Basics of Dirichlet-based models}
  In this section, we introduce the basics of Dirichlet-based models for classification tasks. To ease the introduction, let us start by considering a training dataset \(D = \{x_i, y_i\}_{i = 1}^N\), where \(N\) denotes the total number of data points in the dataset. We assume that labels \(y_i\) belong to one of the \(K\) classes.% in the classification problem.

  Typically, the Dirichlet-based approaches assume that the model consists of two hierarchical random variables, \(\muv\) and \(\theta\). The posterior predictive distribution for a given unseen object \(x\) can be computed as follows:
  %\mt{a diagram could be helpful here?? // MP: probably yes but not absolutely necessary (and no time to plot)}
  \begin{equation*}
    p(y \mid x, D) = \int p(y \mid \muv) \Bigg[\int p(\muv \mid x, \theta) ~ p(\theta \mid D) d\theta \Bigg] d \muv,
  \end{equation*}
  where \(p(y \mid \muv)\) is the distribution over class labels, given some probability vector (e.g., Categorical), \(p(\muv \mid x, \theta)\) is the distribution over a simplex (e.g., Dirichlet), and \(p(\theta \mid D)\) is the posterior distribution over parameters over the model.

  However, for practical neural networks, the posterior distribution \(p(\theta \mid D)\) does not have an analytical form and is computationally intractable. Following~\cite{malinin2018predictive}, we suggest considering ``semi-Bayesian'' scenario by looking on a point estimate of this distribution: \(p(\theta \mid D) = \delta(\theta - \hat{\theta})\), where \(\hat{\theta}\) is some estimate of the parameters (e.g., MAP estimate). Then the integral inside the brackets simplifies:
  %\mt{in the formulation above, there is "not really an integral in the bracket", maybe we could move the first $\int$ inside? Clear to me, but not to reviewer \# 2}
  \begin{equation*}
    \int p(\muv \mid x, \theta) ~ p(\theta \mid D) d\theta = \int p(\muv \mid x, \theta) ~ \delta(\theta - \hat{\theta}) d\theta = p(\muv \mid x, \hat{\theta}).
  \end{equation*}
  %where it is assumed that \(p(\muv \mid x, \hat{\theta}) = \dirplain\) is a Dirichlet distribution. 
  %
  In the series of works~\cite{malinin2018predictive, malinin2019reverse, charpentier2020posterior, charpentier2021natural} the posterior distribution \(p(\muv \mid x, \hat{\theta})\) is chosen to be the Dirichlet distribution \(\dirpost\) with the parameter vector \(\apost(x) = \apost(x \mid \hat{\theta})\) that depends on the input point \(x\). %Before observing any datapoints, we introduce a prior over the class labels.
  In these models, the prior over probability vectors \(\muv\) takes the form of a Dirichlet distribution, representing the distribution over our beliefs about the probability of each class label. In other words, it is a distribution over distributions of class labels. This prior is parameterized by a parameter vector \(\aprior\), where each component \(\apriorc_c\) corresponds to our belief in a specific class.
  % 
  \texttt{PostNet}~\cite{charpentier2020posterior} and \texttt{NatPN}~\cite{charpentier2021natural} propose the idea that the posterior parameters \(\apost(x)\) can be computed in the form of pseudo-counts, parameterized by a function:
  \begin{equation}
  \label{eq:update_rule}
    \apost(x) = \aprior + \al(x),
  \end{equation}
  where \(\al(x) = \al(x \mid \hat{\theta})\) is a function of input object \(x\) that maps it to positive values.% The underlying concept behind these methods is to predict individual posterior updates, as if we had observed a dataset.

  % Given the conjugate relationship between the multinomial likelihood (used for classification) and the Dirichlet prior, we can determine the parameters of the posterior distribution after observing the dataset:
  % \begin{equation*}
  %   \apostc_c = \apriorc_c + \sum_{i = 1}^N \indicator[y_i = c].
  % \end{equation*}
  % %
  % The parameters of the posterior distribution are updated based on the evidence of objects collected from the training dataset.

\paragraph{Parameterization of \(\al(x)\).}
  % In this section we will abuse the notation, ingoring feature extractor. One can think about \(x := g(x)\).

  In \texttt{NatPN}  it is proposed to use the following parameterization: % (we omit parameters indices here for simplicity):
  \begin{equation}
    \al(x) = p\bigl(\embedmodel(x)\bigr) \smmodel\bigl(\embedmodel(x)\bigr).
  \end{equation}
  %
  In this parameterization, \(g(x)\) represents a feature extraction function that maps the input object \(x\) (usually high-dimensional) to a lower-dimensional embedding. 
  Subsequently, \(p(\cdot)\) is a ``density'' function (parameterized by normalizing flow in the case of~\cite{charpentier2021natural, charpentier2020posterior}), and \(\smmodel(\cdot)\) is a function mapping the extracted features to a vector of class probabilities.

  This parameterization offers several advantages. Firstly, since \(p(\cdot)\) is expected to represent the density of training examples, it should be high for in-distribution data. Secondly, as the density is properly normalized, embeddings that lie far from the training ones will result in lower values of \(p\bigl(g(x)\bigr)\), thus leading to lower \(\al(x)\). This means that for such input \(x\), we will not add any evidence, and consequently, \(\apost(x)\) will be close to \(\aprior\).


\subsection{Uncertainty measures for Dirichlet-based models}
\label{sec:uncertainty_measures}
  One of the advantages of using Dirichlet-based models is their ability to easily disentangle and quantitatively estimate aleatoric and epistemic uncertainties.

\paragraph{Epistemic uncertainty.}
  We begin by discussing epistemic uncertainty, which can be estimated in multiple different ways~\cite{malinin2020uncertainty}. %Note, that detailed derivations of these resulting equations are provided in Supplementary Material (SM), Section~\ref{sec:app_uncerainty_measures}.
  In this work, following the ideas from~\cite{malinin2018predictive}, we quantify the epistemic uncertainty as the entropy of a posterior Dirichlet distribution, which can be analytically computed as follows
  \begin{equation}
    \entropy \Big[\dirpost \Big] = \ln\frac{\prod_{i = 1}^K \Gamma\bigl(\apostc_i(x)\bigr)}{\Gamma\bigl(\apostc_0(x)\bigr)} - \sum_{i = 1}^K  \bigl(\apostc_i(x) - 1\bigr) \Bigl(\psi\bigl(\apostc_i(x)\bigr) - \psi\bigl(\apostc_0(x)\bigr)\Bigr),
  \label{eq:entropy}
  \end{equation}
  where \(\apost(x) = \bigl[\apostc_1(x), \dots, \apostc_K(x)\bigr]\) and \(\apostc_0(x) = \sum_{i = 1}^K \apostc_i(x)\).
  
  % Another approach, introduced in~\cite{malinin2018predictive}, is based on the mutual information (MI) between class labels and the categorical distribution, parametrized by the predicted Dirichlet. This can also be computed analytically:
  % \begin{equation*}
  %   MI[y, \muv \mid \apost(x), D] =  
  %   -\sum_{i = 1}^K \frac{\apostc_i(x)}{\apostc_0(x)} \biggl[\ln\frac{\apostc_i(x)}{\apostc_0(x)} - \psi\bigl(\apostc_i(x) + 1\bigr) + \psi\bigl(\apostc_0(x) + 1\bigr) \biggr].
  % \end{equation*}
  % %
  % Both of these metrics measure the width of the resulting Dirichlet distribution, and thus can be considered as a ``measure of disagreement'' between elements of an ensemble formed by sampling from this Dirichlet.

  % \mt{not a nice transition to this sentence // MP: I agree we will rewrite it once we see what measures are more useful}
  % Finally, in~\cite{malinin2020uncertainty}, two additional measures of epistemic uncertainty were introduced. The first one is the Expected Pairwise Kullback-Leibler divergence (EPKL). This measure can also be computed analytically and is formally defined as (see SM, Section~\ref{sec:app_uncerainty_measures}):
  % \begin{equation*}
  %   K[y, \muv \mid \apost(x), D] =
  %   \sum_{i = 1}^K \frac{\apostc_i(x)}{\apostc_0(x)} \biggl[\psi\bigl(\apostc_i(x) + 1\bigr) - \psi\bigl(\apostc_0(x) + 1\bigr) - \psi\bigl(\apostc_i(x)\bigr) + \psi\bigl(\apostc_0(x)\bigr)\biggr],
  % \end{equation*}
  % where both later terms can be computed analytically using the properties of the Dirichlet distribution.

  % The second measure is Reverse Mutual Information (RMI)  (see SM, Section~\ref{sec:app_uncerainty_measures})
  % \begin{equation*}
  %   RMI[y, \muv \mid \apost(x), D] = \sum_{i = 1}^K \frac{\apostc_i(x)}{\apostc_0(x)} \biggl[\ln\frac{\apostc_i(x)}{\apostc_0(x)} - \psi\bigl(\apostc_i(x)\bigr) + \psi\bigl(\apostc_0(x)\bigr) \biggr],
  % \end{equation*}
  % which can also be computed analytically. As demonstrated in~\cite{malinin2020uncertainty}, these last three measures of epistemic uncertainty are related by the following equation:
  % \begin{equation*}
  %   RMI[y, \muv \mid \apost(x), D] = K[y, \muv \mid \apost(x), D] - MI[y, \muv \mid \apost(x), D].
  % \end{equation*}
  % %
  % It is essential to recognize that all these metrics measure the disagreement between ``ensembles'' formed by samples from the posterior Dirichlet distribution. Consequently, there are no inherently correct or incorrect formulas; each of them estimates epistemic uncertainty from a different perspective.

  \paragraph{Aleatoric uncertainty.} Aleatoric uncertainty can be measured using the average entropy~\cite{kendall2017uncertainties}, which can be computed as follows:
  \begin{equation}
    \E_{\muv \sim \dirpost} \entropy[p(y \mid \muv)] = -\sum_{i=1}^K \frac{\apostc_i(x)}{\apostc_0(x)} \biggl[\psi\bigl(\apostc_i(x) + 1\bigr) - \psi\bigl(\apostc_0(x) + 1\bigr)\biggr].
\label{eq:expected_entropy}
  \end{equation}
  %
  This metric captures the inherent noise present in the data, thus providing an estimate of the aleatoric uncertainty.

  In the next section we are going to show how Dirichlet-based models and uncertainty measures based on them can be used in federated learning scenario.

\section{FedPN: \texttt{NatPN} goes federated}
  %We choose to utilize the \texttt{NatPN} model among other Dirichlet-based models for several reasons. First, it does not require explicit out-of-distribution data during training. Second, the idea of using normalizing flows to approximate the density of training data ensures that the density will be low for out-of-distribution data (due to the normalization of the density). Consequently, we will automatically assign low evidences to out-of-distribution objects, which is consistent with the overall intuition.

  %Following \texttt{NatPN}, we begin with the introduction of a feature extractor -- a deep neural network, parametrized by parameters \(\phi\), \(\embedmodel_\phi\colon \R^d \to \R^m\), where \(m\) is the dimensionality of the embedding space. %and \(m < d\). 
  Suppose we are given an array of datasets \(D_i\) for \(1 \leq i \leq b\), where \(b\) represents the number of clients. Each \(D_i = \{x^i_j \in \R^d, y^i_j\}_{j = 1}^{|D_i|}\) consists of object-label pairs. We construct our federated framework in such a way that all clients share the feature extractor $g$ parameters \(\phi\) and maintain personalized heads $f^i$ parameterized by \(\theta_i\).
  % Moreover, we will also keep ``global model'', which is simply the average of personal models: \(\theta = \frac{1}{b}\sum_{i=1}^b \theta_i\).
  Furthermore, we retain a ``global'' head-model $f$, which is trained using the \texttt{FedAvg}~\cite{mcmahan2017communication} (and \texttt{SCAFFOLD}~\cite{karimireddy2020scaffold}) method and which ultimately has parameters \(\theta\).

  Following the \texttt{NatPN} approach, we employ normalizing flows to estimate the embedding density.
  As it is for head models, here we also learn two types of models -- a local density models $p^i$ (using local data) parameterized by $\psi_i$ and global density model $p$ (using data from other clients in a federated fashion) parameterized by $\psi$.
  It is important to note that both types of models are trained on the same domain since the feature extractor model is fixed for local and global models.

  The loss function used in~\cite{charpentier2021natural, charpentier2020posterior} is the expected cross-entropy, also known as Uncertain Cross Entropy (UCE)~\cite{bilovs2019uncertainty}. Note, that this loss function is a \textit{strictly proper scoring rule}, which implies that a learner is incentivized to learn the true conditional \(p(y \mid x)\). For a given input \(x\), the loss can be written as:
  \begin{multline}
  \label{eq:expected_ce}
    L(y, \apost(x)) = \E_{\muv \sim \dirpost} \sum_{i=1}^K -\indicator[y = i]\log\mu_i d\muv =
    %-\E_{\muv \sim \dirpost}\log\mu_y d\muv =
    \psi\bigl(\apostc_0(x)\bigr) - \psi\bigl(\apostc_y(x)\bigr),
  \end{multline}
  where \(\apostc_0(x) = \sum_{i=1}^K \apostc_i(x)\). Additionally, authors suggest to penalize too concentrated predictions, by adding the regularization term with some hyperparameter \(\lambda\). The overall loss function looks as follows:
  \begin{equation}
  \label{eq:bayesian_loss}
    L\bigl(y, \apost(x)\bigr) - \lambda\entropy\bigl[\dirpost\bigr],
  \end{equation}
  where \(\entropy\) denotes the entropy of a distribution. This overall loss function referred by authors as Bayesian loss~\cite{charpentier2021natural, charpentier2020posterior}.


\paragraph{Issues with loss functions.} 
  Let us explore an asymptotic form of~\eqref{eq:expected_ce}.
  For all \(x>0\), the following inequality holds:
  \begin{equation*}
    \log x - \frac{1}{x} \leq \psi(x) \leq \log x - \frac{1}{2x}.
  \end{equation*}
  %
  Recalling the update rule~\eqref{eq:update_rule} and using the specific parameterization of \(\apriorc_c = 1\) for all \(c\), we conclude that all \(\apostc_c(x) > 1\).
  Hence, we can approximate \(\psi\bigl(\apostc_c(x)\bigr) \approx \log \apostc_c(x)\).

  To simplify the notation, we will use \(z = g(x)\):
  \begin{equation} \label{eq:loss_decomposition}
    L\bigl(y, \apost(x)\bigr) \approx \log \bigl(\apostc_0(x)\bigr) - \log \bigl(\apostc_y(x)\bigr)
    = \log K + \log \left[ 1 + \frac{p(z) \left(\frac{1}{K} - f_y(z)\right)}{\apriorc_y + p(z)f_y(z)} \right],
  \end{equation}
  see the full derivation in Supplementary Material (SM), Section~\ref{sup:loss}.

  We observe from~\eqref{eq:loss_decomposition} that for an in-distribution case with high aleatoric uncertainty (when all classes are confused and equally probable), the last term is canceled.
  Note, that the presence of entropy term (that is used in~\cite{charpentier2021natural, charpentier2020posterior} resulting to the final loss of equation~\eqref{eq:bayesian_loss}), which incentives learner to produce smooth prediction will only amplify the effect.
  This implies that no gradients concerning the parameters of the density model will be propagated.
  As a result, \(p(\cdot)\) may disregard regions in the embedding space that correspond to areas with a high concentration of ambiguous training examples.
  This \textit{violates the intuition of \(p(\cdot)\) as a data density}. Thus, uncertainty estimates based on \(p(\cdot)\) cannot be used to measure epistemic uncertainty, as it ignores the regions with high aleatoric uncertainty. %The correct treatment of \(p(z)\) in that case would be as the \textit{confidence} of the model in the prediction at a particular \(x\), rather than density.

  \begin{figure}[t!]
    \centering
    \begin{subfigure}{0.32\textwidth}
      \includegraphics[width=\linewidth]{pics/digamma_loss_K=10.pdf}
    \end{subfigure}
    \hfill
  %   \begin{subfigure}{0.45\textwidth}
  %     \includegraphics[width=\linewidth]{pics/digamma_loss_K=1000.pdf}
  %   \end{subfigure}
  %   \caption{Images depict the landscape of the loss function with varying predicted probabilities for the correct class. \textbf{Left:} With  \(K=10\) classes, the red line (representing high aleatoric regions) appears relatively flat. Even at this level, the density in corresponding points tends to be underestimated. As the number of classes increases, this effect is amplified. \textbf{Right:} When \(K = 1000\), the red line becomes even flatter, exacerbating the issue. Interestingly, for outlier points, the loss function actually reduces the mass on these points, contrasting with the intuitive expectation of fitting the density of the training data.}
  %   \label{fig:ce_loss_issue}
  % \end{figure}
  %
  % \begin{figure}[t!]
  %   \centering
    \begin{subfigure}{0.32\textwidth}
      \includegraphics[width=\textwidth]{pics/toy_example_illustrative.pdf}
    \end{subfigure}
    \hfill%\hspace{0.05\textwidth} % Horizontal space between the two figures
    \begin{subfigure}{0.32\textwidth}
      \includegraphics[width=\textwidth]{pics/mid_mode_density_degradating.pdf}
    \end{subfigure}
    \caption{\textbf{Left:} Image depicts the landscape of the loss function with \(K=10\) classes. The red line (representing high aleatoric regions) appears relatively flat. Even at this level, the density in corresponding points tends to be underestimated. As the number of classes increases, this effect is amplified. \textbf{Center:} This image depicts the training data, where the leftmost and rightmost Gaussians consist of only one class each. In contrast, the middle Gaussian contains all \(K\) labels, randomly permuted. Each Gaussian has an equal number of data points, implying that, if \(p(z)\) follows the intuition of density, all peaks should have the same height. \textbf{Right:} By altering the number of classes \(K\), we change the aleatoric uncertainty. We train the model using the vanilla approach of \texttt{NatPN} and measure \(p(z)\) at the central peak. As the number of classes increases, the density decreases, violating the intuition that \(p(z)\) is the density of training data.}
    \label{fig:toy_illustration}
  \end{figure}

  In addition to the problem of confusing high-aleatoric and high-epistemic regions, we discovered that the proposed loss function defy intuition when confronted with ``outliers.'' We define an ``outlier'' as an object with a predicted probability less than \(\frac{1}{K}\). From~\eqref{eq:loss_decomposition}, we observe that
  %when all \(\apriorc_c = 1\) (following~\cite{charpentier2021natural, charpentier2020posterior}),
  the last term changes its sign precisely at the point where \(f_y(z) = \frac{1}{K}\). This implies that to minimize the loss function, we must decrease \(p(z)\) at these points, which seems counterintuitive since these \(z\) values correspond to objects from our training data.

  Although the issue concerning equation~\eqref{eq:expected_ce} arises primarily in the asymptotic context, we can readily illustrate it through the loss function profiles (see Figure~\ref{fig:toy_illustration}-left) for a range of fixed correct class prediction probabilities.

  To further emphasize the problem, we examine the loss function landscape and provide a demonstrative example. Consider three two-dimensional Gaussian distributions, each with a standard deviation of \(0.1\) and means of -1, 0, and +1 with respect to the first coordinate, while the second coordinate of the mean is equal to \(0\) for all three clusters (see Figure~\ref{fig:toy_illustration}-center). Left and right clusters are set to include objects of only one class, while the middle distribution contains uniformly distributed labels, representing a high aleatoric region. Each Gaussian contains an equal amount of data. We train the \texttt{NatPN} model using a centralized approach, employing the loss function from equation~\eqref{eq:expected_ce}. Subsequently, we evaluate the quality of the learned model by plotting the density in the center of middle Gaussian. Ideally, we would expect three peaks of equal size, and the density of the middle Gaussian stay constant with the number of classes \(K\). However, we observe the different picture with ``density'' estimate at the central cluster decreasing when one increases the number of clusters, see Figure~\ref{fig:toy_illustration}-right.

  It is essential to emphasize that addressing these issues is critical for our framework, as we need to accurately differentiate between aleatoric and epistemic uncertainties in order to select the appropriate model for a given situation.
  Consequently, in the following section, we propose a simple but efficient technique to rectify the aforementioned problem with the loss function, ensuring that our framework effectively distinguishes between the different types of uncertainties and makes informed model choices.


\paragraph{Proposed solution.} We propose to still use parametric model to estimate density, but now our goal is to ensure that \(p(\cdot)\) accurately represents the density of our training embeddings. To achieve this, we propose maximizing the likelihood of the embeddings explicitly by incorporating a corresponding term into the loss function.
  Simultaneously, we aim to prevent any potential impact of the Bayesian loss on the density estimation parameters, maintaining their independence.

  Thus, we suggest the following loss function:
  \begin{equation}
    L\bigl(y, \text{StopGrad}_{p(\embedmodel(x))} \apost(x)\bigr) - \lambda\entropy\bigl[\dirpost\bigr] - \gamma \log p\bigl(\embedmodel(x)\bigr),
  \end{equation}
  where \(\lambda, \gamma > 0\) are hyperparameters, and \(\text{StopGrad}_{p(\embedmodel(x))}\) means that the gradient will be not propagated to the parameters of a density model, which parameterizes \(p\bigl(\embedmodel(x)\bigr)\).


==> neurips_2023/related_work.tex <==
\section{Related Work}
\label{sec:related_work}
\todo[inline,color=pink]{shall we put this a bit sooner?}
The problem of uncertainty quantification has been extensively studied in numerous centralized scenarios across various data domains. However, the application of this topic to federated learning has not yet been thoroughly investigated. While some attempts have been made to quantify uncertainty in federated settings, such as in~\cite{linsner2022approaches, kotelevskii2022fedpop}, these studies neither differentiate between aleatoric and epistemic uncertainties nor provide practical solutions.

In~\cite{linsner2022approaches}, the authors suggest training an ensemble of $K$ global models as the best approach, which is $K$ times more expensive compared to the classical \texttt{FedAvg} method. In~\cite{kotelevskii2022fedpop}, the authors propose using Markov Chain Monte Carlo (MCMC) to obtain samples from the posterior distribution, which is practically almost infeasible due to its computational complexity.

Other works, such as~\cite{chen2020fedbe, kimhierarchical}, could potentially be utilized for estimating uncertainty in federated learning. However, these studies do not explicitly discuss the opportunities and challenges associated with uncertainty quantification in their papers.

Consequently, our paper stands out as one of the few studies that specifically addresses the problem of uncertainty quantification in federated learning. We aim to provide a comprehensive analysis of this important topic, considering both theoretical and practical aspects, and presenting solutions that overcome the limitations of existing approaches in the literature.

==> sections/related_work.tex <==
% !TEX root = ../main.tex

\section{Related Work}
\label{sec:related_work}
\todo[inline,color=pink]{shall we put this a bit sooner?}
The problem of uncertainty quantification has been extensively studied in numerous centralized scenarios across various data domains. However, the application of this topic to federated learning has not yet been thoroughly investigated. While some attempts have been made to quantify uncertainty in federated settings, such as in~\citep{linsner2022approaches, kotelevskii2022fedpop}, these studies neither differentiate between aleatoric and epistemic uncertainties nor provide practical solutions.

In~\citep{linsner2022approaches}, the authors suggest training an ensemble of $K$ global models as the best approach, which is $K$ times more expensive compared to the classical \texttt{FedAvg} method. In~\citep{kotelevskii2022fedpop}, the authors propose using Markov Chain Monte Carlo (MCMC) to obtain samples from the posterior distribution, which is practically almost infeasible due to its computational complexity.

Other works, such as~\citep{chen2020fedbe, kimhierarchical}, could potentially be utilized for estimating uncertainty in federated learning. However, these studies do not explicitly discuss the opportunities and challenges associated with uncertainty quantification in their papers.

Consequently, our paper stands out as one of the few studies that specifically addresses the problem of uncertainty quantification in federated learning. We aim to provide a comprehensive analysis of this important topic, considering both theoretical and practical aspects, and presenting solutions that overcome the limitations of existing approaches in the literature.

